Discovery of two little red dots transitioning into quasars

James Webb Space Telescope (JWST) has uncovered a new population of compact objects that show a unique V-shaped spectral energy distribution (SED) in the UV and optical wavelength range. These so-called "little red dots" (LRDs) often exhibit broad Balmer emission lines, indicative of the presence of active galactic nuclei (AGNs). They generally lack detection of X-ray, radio, and mid-IR radiation, which is fundamentally different from typical AGNs. Various models, including super-Eddington-accreting black holes enshrouded in dense and dust-poor gas, have been proposed to explain these features. However, the nature of LRDs remains debated, and their evolutionary fate is unclear. Here we report two unusual LRDs at redshift z = 2.868 and 2.925 that are in a transitional phase towards typical AGNs. Their V-shaped SEDs, compact optical morphology, and broad emission lines satisfy the defining criteria of LRDs. On the other hand, they exhibit intense X-ray, radio, and mid-IR radiation that is much stronger than previously known LRDs. These hybrid properties suggest that the dense gas envelope around their central black holes is dispersing, allowing high-energy photons and radio emission to escape. Meanwhile, a dust torus is forming. This finding provides a direct insight into the nature of LRDs and indicates that at least some LRDs will evolve into AGNs or quasars at later times.

==> deprecated_part.tex <==
\medskip
% PSF SED modeling （+Mid-IR）
From morphological decomposition, we find that the PSF becomes increasingly dominant from the UV–optical to the NIR for the \textit{Forges}.
At wavelengths longer than F444W (JWST/MIRI and Spitzer), the mid-IR emission of the \textit{Forges} is stronger than that of high-redshift LRDs.  The sources appear point-like in JWST/MIRI and Spitzer, albeit at lower resolution than JWST/NIRCam. Therefore, we attribute the emission entirely to the central source.  
The optical–IR SEDs of the central point sources can then be well reproduced by the super-Eddington accretion model from ref.\cite{LiuH_2025}, supplemented by two additional blackbody components with characteristic temperatures of $T \sim 500$\,K and $T \sim 1500$\,K (Extended Data Figure \ref{fig:SED}). In this framework, optically thick photospheres around the super-Eddington accreting black hole with a characteristic effective temperature of $\sim 5000$\,K naturally generate both the red optical continua and the Balmer break\cite{LiuH_2025}, while the dust components can be interpreted as emission from an emerging torus. 
There are indications that low-redshift LRDs exhibit enhanced IR emission compared with their high-redshift counterparts (Fig. B.1 of \cite{2025arXiv250907100D}), suggesting that our sources likely represent a more evolved and mature stage relative to high-redshift LRDs.
%a clumpy torus structure in formation\cite{2024MNRAS.535..853J}.  
\medskip
% host SED fitting
%Assuming that all extended emission in the high-resolution NIRCam images of the \textit{Forges} originates from the host galaxies, 
We model the SEDs of the host galaxies of the \textit{Forges} using the SED-fitting code \texttt{CIGALE} (v2025; \cite{2005MNRAS.360.1413B,2019A&A...622A.103B}), incorporating the flux of the extended component obtained from decomposed JWST/NIRCam images, together with lower-resolution data at wavelengths blueward of NIRCam. The star formation rates (SFRs) of the \textit{Forges} inferred from SED modeling are $12.9 \pm 6.6\  M_\odot\,\rm{yr}^{-1}$ and $62.8 \pm 10.3\ M_\odot\,\rm{yr}^{-1}$, with corresponding stellar masses of $\log (M_\ast/M_\odot)=9.14 \pm 0.19$ and  $\log (M_\ast/M_\odot)=10.31 \pm 1.38$, respectively, placing them on the star-forming main sequence at $z \sim 3$\cite{Santini_2017,Clarke_2024}.  As shown in the left panel of Figure~\ref{fig:MBH_Ms}, the \textit{Forges} fall in between the parameter space of LRDs and luminous quasars in terms of black hole and host stellar masses. 
Other physical properties derived from SED modeling are listed in Table~\ref{tab:bh_properties}. 
There is a distinct 2175\,\AA\ absorption feature in their rest-frame UV SEDs (Extended Data Figure~\ref{fig:SED}), pointing to the presence of graphitic dust grains\cite{Sorrell_1990, 2021ApJ...909..213K}. 
\medskip
% model nebular emission
About $30\%$ of LRDs exhibit off-centered, extended emission\cite{2024arXiv241114383R}. Previous works proposed that such off-centered emission could arise from nebular emission powered by the central AGN \cite{Chen2025b}, rather than by ionization from young stars.
In The Forges, the off-centered emission is particularly strong in the F200W and F277W bands, corresponding to the wavelength ranges of [\ion{O}{III}]/H$\beta$ and H$\alpha$, indicating a potentially non-stellar source of ionization. We fit the SEDs of the off-centered Sérsic components by modeling them as nebular gas photoionized by the central AGN (Method). In this framework, a fraction of the UV emission is absorbed by the optically thick photospheres and reprocessed into blackbody radiation with a characteristic effective temperature of ∼5000 K, while the remaining ionizing photons escape through the open angle to photoionize the surrounding nebula.
%It has been proposed that at least part of the off-centered emission in LRDs could arise from nebular emission powered by the central AGN \cite{Chen2025b}, rather than by ionization from the young stellar component. However, Our morphological decomposition reveals a decline in the point-source contribution from the rest-frame NIR to the optical–UV, suggesting that the central source does not provide sufficient ionizing photons to power the nebular emission. The galaxy model alone is sufficient to reproduce the UV SED, indicating that the galaxy dominates the ionizing UV SED, which is also supported by the non-detections of high-ionization UV emission lines of AGN.




\textbf{To be discussed...} 
Based on previous studies, the red optical color, weak X-ray emission, low UV-optical variability, Balmer absorption lines, and Balmer break of LRDs may be explained by super-Eddington accreting black holes enshrouded in extremely dense gas ($n_{\rm H} \sim 10^{9}$--$10^{11}\,\rm cm^{-3}$)\cite{2024A&A...691A.145M,2025ApJ...980L..27I,Lin2025_locallrd}, while the blue UV emission possibly arises from the spatially extended, less-obscured host galaxy\cite{2024ApJ...969L..13W,2024A&A...691A..52K,Kocevski2025} or nuclear young stellar population\cite{2025arXiv250919422I}.
In this work, our results point toward a possible physical picture in which the \textit{Forges} are transitional systems: LRDs caught in the act of becoming quasars. As shown in the right panel of Figure~\ref{fig:MBH_Ms}, the \textit{Forges} are offset from the bulk of the LRD population and already share comparable $L_{\rm bol}$ and $M_{\rm BH}$ with quasars at lower redshift. The presence of \ion{O}{i} $\lambda 11287$ emission and strong X-ray variability implies they are still super-Eddington accreting. The host galaxies are already well assembled, while their SFRs remain high, therefore they are approaching the local scaling relation. 
Previously, there were only two X-ray-detected LRDs reported \cite{Kocevski2025} (with redshift of 4.66 and 3.1), where X-ray spectral analysis confirms that the AGN are moderately obscured. Similarly, in those sources, they suggest a reddened AGN emission dominates the rest-optical light, while the rest-UV emission originates from the host galaxy. 
In the main population of LRDs, most of which are at high redshift ($z\gtrsim4$)\cite{Labbe2023,Matthee2024,Akins2024a_cos}, X-ray-weak and IR-weak sources are embedded within dense gas envelopes, which suppress the escape of X-ray photons\cite{LiuH_2025,Lin2025_locallrd,2025arXiv250506965K}.
In the \textit{Forges} and the previous X-ray-detected LRDs, we are likely witnessing the destruction of the gas envelope surrounding the black hole, possibly leading to a clumpy and porous structure with occasional low-density paths. The emerging X-ray emission can escape while most UV photons remain trapped, owing to the much smaller cross-section of X-rays and/or a smaller X-ray emission region. Jets are weakly confined, giving rise to the observed radio emission. At the same time, graphite dust grains formed by circumnuclear starbursts, as indicated by the strong 2175~\AA\ absorption feature in the SED, migrate inward and gradually assemble into a clumpy torus. 
At this stage, different viewing angles yield distinct observational properties.
%Based on the steep radio spectral indices of the \textit{Forges}, we are likely viewing both systems edge-on, with the redshifted \ion{He}{i} absorption tracing the inward motion of the forming torus. 
Eventually, the \textit{Forges} may evolve into classical AGN, where the torus is fully formed.
In this sense, the \textit{Forges} provide a natural link between the compact, red, enigmatic LRDs and the luminous AGN population that dominates cosmic accretion power at later times.


